Image Protection for Robust Cropping Localization and Recovery

Existing image cropping detection schemes ignore that recovering the cropped-out contents can unveil the purpose of the behaved cropping attack. This paper presents \textbf{CLR}-Net, a novel image protection scheme addressing the combined challenge of image \textbf{C}ropping \textbf{L}ocalization and \textbf{R}ecovery. We first protect the original image by introducing imperceptible perturbations. Then, typical image post-processing attacks are simulated to erode the protected image. On the recipient's side, we predict the cropping mask and recover the original image. Besides, we propose a novel \textbf{F}ine-\textbf{G}rained generative \textbf{JPEG} simulator (FG-JPEG) as well as a feature alignment network to improve the real-world robustness. Comprehensive experiments prove that the quality of the recovered image and the accuracy of crop localization are both satisfactory.

==> related_works.tex <==
% \subsection{Image extrapolation.} 
% Image extrapolation (or out-painting)~\cite{wang2021rego,wang2021sketch,cheng2021out, van2019image} is a famous perceptual-driven image recovery technology that can extend the image borders. These schemes usually employ a searching pipeline~\cite{cheng2021out, van2019image} for plausible structure and details, or rely on extra guidance such as a sketch~\cite{wang2021sketch} or a reference~\cite{wang2021rego}. 
% For example, Van et al.~\cite{van2019image} proposes the first GAN-based method for image outpainting, and Chen et al.~\cite{cheng2021out} employs GAN inversion for higher-quality image outpainting which renders micro-patches conditioned on the predicted latent code as well as their individual positions in the image.
% REGO~\cite{wang2021rego} additionally synthesizes user-friendly output images by introducing a sketch for reference.
% The results look promising, though image outpainting can never faithfully recover the missing information. In contrast, CLR-Net focuses on accurate recovery, and therefore image out-painting is not a good benchmark for comparison.
In this section, we review the related works of the proposed method, namely, image watermarking, image cropping detection \& localization, and invertible networks for data hiding.
\subsection{Image watermarking}
Watermarking~\cite{tao2018towards,wu2020watermarking,ying2021hiding} is an important branch of steganography~\cite{qian2018new,feng2019diversity} which highlights robust and imperceptible information hiding into the host data for covert purposes.
Many traditional image watermarking methods work on different transform domains including Discrete Fourier Transform (DFT)~\cite{cheng2003robust}, Discrete Cosine Transform (DCT)~\cite{wang2006blind,mareen2018scalable}, Discrete Wavelet Transform (DWT)~\cite{lai2010digital,liu2020discrete} and Dual-Tree Complex Wavelet Transform (DTCWT)~\cite{ying2019robust,wang2022dtcwt}.
With the emergence of deep learning, there exists a number of deep-network-based watermarking methods~\cite{shin2017jpeg,zhu2018hidden,liu2021jpeg}. 
An encoder is usually employed to transform the original images into marked images, and a decoder extracts the hidden message from the received image.
To enable robustness, these schemes usually follow a multi-task learning agenda where in each iteration the algorithms add a selected kind of attack on the marked images. The attacks are implemented by an attack layer using differentiable methods. 
However, different image post-processing attacks share varied characteristics, and such techniques can potentially lead to unbalanced robustness.
% The gradients of the network can be much larger when weaker attacks are involved. As a result, 
% the networks can over-fit weak attacks but perform poorly against heavy attacks. 
% We propose to apply image pre-processing on the attacked image ahead of the downstream task to alleviate this problem.

% Besides, many schemes still lack real-world robustness against JPEG compression.
% Previous researches have proposed several mask-based JPEG simulator~\cite{shin2017jpeg,zhu2018hidden,liu2021jpeg}. In these schemes, JPEG compression is simulated step by step using \greenmarker{a} differentiable methods, where quantization is conducted using differentiable rounding function~\cite{bengio2013estimating} and a pre-defined quantization table. However, the hand-crafted quantization tables in these schemes are immutable, which is in contrast with the quantization table in real-world JPEG images that can be customized and flexibly controlled by the quality factor as well as the image content. As a result, the neural networks can over-fit and lack real-world robustness. We present the novel FG-JPEG based on generative networks to allow more flexibility in the simulation.

% \subsection{Image protection using watermarking}
Many fragile watermarking schemes for image self-recovery have been proposed. 
He et al.~\cite{he2006wavelet} embed the shuffled DCT coefficients into the Least Significant Bit (LSB) planes of the host image. As a result, after data extraction by the recipient, he can only recover a blurry version of the original image. 
Zhang et al.~\cite{zhang2008fragile} propose to embed into the image blocks check-bits and reference-bits, where the former identifies the tampered blocks and the latter can exactly reconstruct the original image.
% Zhang et al.~\cite{zhang2011self} \redmarker{propose} an improved scheme where the watermark data are embedded into the LSB planes, produced by exclusive-or operation on the original Most Significant Bits (MSBs) of a pair of pixels. 
% Zhang et al.~\cite{zhang2010reference} \redmarker{propose} a reference sharing mechanism for improved content recovery. 
Korus et al.~\cite{korus2012efficient} theoretically analyze the reconstruction performance with the use of communication theory.
But these methods are fragile and not developed for image cropping recovery.
Our previous work named Imuge~\cite{ying2021image} presents a robust watermarking scheme that protects images from being maliciously manipulated. After the recipient gets the tampered protected image, he can conduct accurate tamper localization and image recovery.
% The method is proven to have strong robustness against typical image processing attacks and shows promising results in both tamper localization and content recovery.
What's more, there are some works that use watermarking for the prevention of image inpainting~\cite{khachaturov2021markpainting} or super-resolution (SR)~\cite{yin2018deep}.
% In~\cite{khachaturov2021markpainting}, the authors propose a watermarking-like adversarial method, call markpainting, making an in-painting system into generating a patch similar to an arbitrary target. It makes input image robust against watermark removal by adding minor perturbations to the images. In~\cite{yin2018deep}, the authors propose an adversarial attack method to cause errors in super-resolution model, including making the SR image has undesired style, be incorrectly classified in classification task, or generates wrong words in image caption task. 

However, none of the above-mentioned works address the issue of image anti-cropping using image cropping recovery. This paper addresses the issue of robust image cropping localization and recovery.

% \subsection{Invertible Neural Networks}
% Invertible neural network (INN)~\cite{dinh2014nice,dinh2016density,grathwohl2018ffjord,kingma2018glow} learns a stable invertible mapping from the source distribution $\mathcal{P}_{s}$ to a targeted distribution $\mathcal{P}_{t}$, which involves the forward and back propagation operations in the same network.
% INN involves the forward and back propagation operations in the same network, such that it realizes both the feature encoder and the image generator.
% The invertible neural network has attracted much attention, as it is one of the effective schemes for reversible image transformation. 

% INNs are previously used for various low-level computer vision tasks, for example, image colorization~\cite{zhao2021invertible} invertible data hiding network (ISN)~\cite{lu2021large,jing2021hinet,ying2021no}, image rescaling~\cite{xiao2020invertible}, etc. In this paper, we are the first to utilize INN in image crop localization and image recovery from the cropped fragment.

\subsection{Image cropping detection and localization.}
% cropping is a simple yet powerful way to maliciously alter the message of an image. This kind of forgery has historically been less investigated by the forensic community than other image manipulations. The main difficulty is that much less semantic or statistical clue of cropping can be discovered. 
The existing image cropping detection algorithms~\cite{fanfani2020vision,yerushalmy2011digital,li2009passive} mainly focus on predicting whether an image is cropped. They are represented by detecting the exposing evidence of asymmetrical image cropping, e.g., the shift of the image center~\cite{fanfani2020vision}, and the inconsistency of JPEG blocking artifacts~\cite{yerushalmy2011digital,li2009passive}.
Fanfani et al.~\cite{fanfani2020vision} 
propose an automated approach for detecting asymmetrically cropped images, where the shift of the image center with respect to the principal point is used to assess cropping.
Yerushalmy et al.~\cite{yerushalmy2011digital} 
exploit image artifacts that are due to chromatic aberrations as indicators for evaluating image authenticity. The trace is introduced in the acquired image by the optical and sensing systems of the camera. 
Specifically, in \cite{li2009passive}, the block artifact grids (BAGs) are extracted blindly with a new extraction algorithm, and then abnormal BAGs can be detected with a marking procedure as a trail of cropping detection.
In comparison, there are fewer schemes developed for image cropping localization.
Van et al.~\cite{van2020dissecting} investigate the subtle traces that cropping has on the image distribution, and predict the absolute location of image patches. For example, lenses will leave behind certain clues, notably chromatic aberration and vignetting. We previously presented a robust watermarking scheme for image cropping localization~\cite{ying2021no}. 
% A INN-based network hides a watermark inside a targeted image.
The image owner embeds a selected watermark and the recipient can robustly extract the watermark and conduct feature matching to predict the cropping mask. 

However, there are certain issues to be addressed. Van et al.~\cite{van2020dissecting} require the images to be untouched and uncompressed so that the tiny clues are preserved. Otherwise, the scheme cannot find enough trace for cropping localization. For~\cite{ying2021no}, the watermark must be shared with the legal recipient.
In contrast, we present CLR-Net that localizes image cropping and conducts image recovery using robust watermarking. It does not require a shared image as the watermark and has no restriction on the image format or quality. 

% Otherwise, without these constraints, the schemes cannot be applied.

% \textbf{Real-World JPEG simulation. }
% Many previous studies include their design of attack layer~\cite{liu2021jpeg,zhu2018hidden,ying2021no}. However, their robustness against JPEG compression in the real world are still reported to have a visible gap with that in the experiments. In this paper, we propose a novel case-aware generative JPEG simulator (CA-JPEG) to address this issue.

% In summary, the drawbacks of the related works concerning our topic are mainly two-folded. 
% (1) Once an image is cropped, there was no way to know what was originally cropped-out.
% (2) Previous image crop localization schemes are not suitable in real-world application due to their own inevitable constraints.


\subsection{Invertible networks for data hiding}
Invertible neural network (INN) learns a stable invertible mapping from the source distribution $\mathcal{P}_{s}$ to a targeted distribution $\mathcal{P}_{t}$, and the forward and back propagation operations are in the same network.
Pioneering research on INN-based mapping can be seen in NICE~\cite{dinh2014nice} and RealNVP~\cite{dinh2016density}. 
Previously, INNs are successfully applied for various low-level computer vision tasks,e.g., image colorization~\cite{zhao2021invertible}, image rescaling~\cite{xiao2020invertible}, etc. 
Most recently, Lu et al.~\cite{lu2021large} and Jing et al.~\cite{jing2021hinet} both use invertible neural networks based on RealNVP for data hiding and extraction. These works can largely increase the overall payload by hiding multiple images simultaneously.
Xu et al.~\cite{xu2022robust} make the first attempt to robustly hide multiple images into a single container using INN. 
% Inspired by these recent successes, we also build our image cropping recovery scheme upon solving an invertible problem. 



% In this paper, we are the first to utilize INN for crop and tamper localization.
